Computing the Least-core and Nucleolus for Threshold Cardinality Matching Games

Cooperative games provide a framework for fair and stable profit allocation in multi-agent systems. \emph{Core}, \emph{least-core} and \emph{nucleolus} are such solution concepts that characterize stability of cooperation. In this paper, we study the algorithmic issues on the least-core and nucleolus of threshold cardinality matching games (TCMG). A TCMG is defined on a graph $G=(V,E)$ and a threshold $T$, in which the player set is $V$ and the profit of a coalition $S\subseteq V$ is 1 if the size of a maximum matching in $G[S]$ meets or exceeds $T$, and 0 otherwise. We first show that for a TCMG, the problems of computing least-core value, finding and verifying least-core payoff are all polynomial time solvable. We also provide a general characterization of the least core for a large class of TCMG. Next, based on Gallai-Edmonds Decomposition in matching theory, we give a concise formulation of the nucleolus for a typical case of TCMG which the threshold $T$ equals $1$. When the threshold $T$ is relevant to the input size, we prove that the nucleolus can be obtained in polynomial time in bipartite graphs and graphs with a perfect matching.

==> bibliography.tex <==
\bibitem{Deng1999}
Deng, X., Ibaraki, T., Nagamochi, H.: Algorithmic aspects of the
core of combinatorial optimization games. Mathematics of Operations
Research {\bf 24} (1999) 751--766

\bibitem{DengPaPa1994}
Deng, X., Papadimitriou, C. H.: On the complexity of
cooperative solution concepts. Mathematics of Operations Research
{\bf 19} (1994) 257--266

\bibitem{DeFaSu06}
Deng, X, Fang, Q. and Sun, X: Finding nucleolus of flow game. In
{\em Proceedings of the 17th Annual ACM-SIAM Symposium on Discrete
Algorithms (SODA'06)}, pages 124--131, 2006.

\bibitem{Kope}
A. Kopelowitz, Computation of the kernels of simple games and the nucleolus of n-person games, RM-31, Math. Dept.,
DeFaSu06DeFaSu06The Hebre University of Jerusalem, 1967.

\bibitem{Maschler}
Maschler, M.; Peleg, B.; and Shapley, L.S.
Geometric propoties of the kernel, nucleolus, and related solution concepts.
Mathematics of Operations Research 4:303--338. 1979

\bibitem{Gillies}
Gillies D B, Some Theorems on n-person Games[D], Ph.D. Thesis.
Prince-ton, New Jersey: Princeton University Press, 1953.
%
\bibitem{Shapley1}
Shapley L S, Shubik M, The core of an economy with nonconvex preferences[R],
RM-3518, The Rand Corporation, Santa Monica, CA, 1963.

\bibitem{Shapley2}
Shapley L S, Shubik M, 
Quasi-cores in a monetary economy with nonconvex preferences[J], 
Econometrica, 1966, 34: 805-827.

\bibitem{Schmeidler}
Schmeidler D, The nucleolus of a characteristic function game[J],
SIAM Jourmal on Applied Mathematics, 1969, 17: 1163-1170.

\bibitem {Sch2003} A. Schrijver, {\em Combinatorial Optimization: Polyhedra and Efficiency.} Springer-Verlag, Berlin Heidelberg,
2003.

\bibitem{Huberman}
G.Huberman, The nucleolus and the essential coalitions,
In: Analysis and Optimizations of Systems, PP, 416-422, Springer, Berlin, 1980.

\bibitem{Haris1}
Haris Aziz, Felix Brandt, Paul Harrenstein.
Monotone cooperative games and their threshold versions.
Proc. of 9th Int. Conf. on Autonomous Agents and Multiagent Systems
(AAMAS2010)

\bibitem{Haris2}
Haris Aziz, Troels B. S.
Path coalitional games.
CoRR, abs/1103.3310, 2011.

\bibitem{Yoram}
Yoram Bachrach, Ely Porat.
Path Disruption Games.
Proc. of 9th Int. Conf. on Autonomous Agents and Multiagent Systems
(AAMAS2010)

\bibitem{Edith}
Edith Elkind, Leslie Ann Goldberg, Paul Goldberg, Michael Wooldridge.
Computation Complexity of Weighted Threshold Games.
Association for the Advancement of Artificial Intelligence(2007)
718--723

\bibitem{Solymosi}
Solymosi, T., and Raghavan, T.
An algorithm for finding the nucleolus of assignment games.
Interntional J. Game Theory 23:119--143 1994

\bibitem{Kern1}
W. Kern, D. Paulusma.
Matching games: The least core and the nucleolus.
2003. Mathmatics of Operation Research 28:294--308

\bibitem{Kern2}
P.B., W. Kern, D. Paulusma.
Computing solutions for matching games.
2012. Int J Game Theory 41:75--90

\bibitem{Ning Chen}
Ning Chen, Pinyan Lu, Hongyang Zhang.
Computing the Nucleolus of Maching, Cover and Clique Games.
Association for the Advancement of Artificial Intelligence(2012)
1319--1325

\bibitem{Douglas}
Douglas B. West.
A short proof of the Berge-Tutte Formula and the Gallai-Edmonds Structure Theorem.
European Journal of Combinatorics(2011)32:674--676

\bibitem{L.Lovasz}
L.Lovasz?????, D.M.Plummer[1986]:Matching Theory.
North-Holland Mathematical Studies vol. 121, Amsterdam.

\end{thebibliography}

